Improving Large-scale Paraphrase Acquisition and Generation

This paper addresses the quality issues in existing Twitter-based paraphrase datasets, and discusses the necessity of using two separate definitions of paraphrase for identification and generation tasks. We present a new Multi-Topic Paraphrase in Twitter (MultiPIT) corpus that consists of a total of 130k sentence pairs with crowdsoursing (MultiPIT_crowd) and expert (MultiPIT_expert) annotations using two different paraphrase definitions for paraphrase identification, in addition to a multi-reference test set (MultiPIT_NMR) and a large automatically constructed training set (MultiPIT_Auto) for paraphrase generation. With improved data annotation quality and task-specific paraphrase definition, the best pre-trained language model fine-tuned on our dataset achieves the state-of-the-art performance of 84.2 F1 for automatic paraphrase identification. Furthermore, our empirical results also demonstrate that the paraphrase generation models trained on MultiPIT_Auto generate more diverse and high-quality paraphrases compared to their counterparts fine-tuned on other corpora such as Quora, MSCOCO, and ParaNMT.

==> fig/distribution.tex <==
\begin{figure*}[t]

\begin{center}

\includegraphics[width=0.195\linewidth]{fig/stage_2_bleu_distribution_count (5).pdf}
\includegraphics[width=0.195\linewidth]{fig/stage_2_bert_distribution_count (4).pdf}
\includegraphics[width=0.195\linewidth]{fig/stage_2_bleu_distribution_bert_71_count (3).pdf}
% \includegraphics[width=0.195\linewidth]{fig/stage_2_bert_distribution_ecdf (5).pdf}
\includegraphics[width=0.195\linewidth]{fig/stage_2_bleurt_distribution_count (2).pdf}
\includegraphics[width=0.195\linewidth]{fig/stage_2_bleu_distribution_bleurt_47_count (2).pdf}
\end{center}

\caption{
Identified paraphrase pairs distributions from various metrics and filtering. BERT-Score or BLEURT filtering is necessary to separate non-paraphrase pairs from paraphrase pairs. Both BERT-Score and BLEURT filtering have similar effect. $71$ and $47$ are the numbers at the max distance between the ECDF of paraphrase and non-paraphrase distributions at BERT-Score and BLEURT respectively. 
}
\label{fig:distrubution}
\end{figure*}

==> fig/encoder_decoder.tex <==
\begin{table*}[t]
\centering
% \renewcommand{\arraystretch}{1.2}
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}lcccccc|cccccc@{}}
    \toprule
    \textit{Test set} $\rightarrow$ & \multicolumn{6}{c}{\textbf{MultiPIT-NMR}} &                                  \multicolumn{6}{c}{\textbf{ParaNMT}} \\
    \cmidrule(r){2-7} \cmidrule(r){8-13}
       \textbf{EncoderDecoder} & BL & R-L & S-B $\downarrow$ & BertScore & BertScore(ref) & B-iB & BL & R-L & S-B $\downarrow$ & BertScore & BertScore(ref) & B-iB   \\ 
       \midrule
       \textit{Fine-tune on M} \\
          BERT\textsubscript{large}-random-init.   & 6.27 & 26.37 & 1.78 & 81.46 (60.32) & 83.58 & 83.82 & 0.18 & 10.36 & 0.35 & 83.88 (53.05) & 83.75 & 86.10\\
        BERT\textsubscript{large}     & 20.86 & 44.71 & 11.81 & 86.35 (72.48) & 87.89 & 86.00 & 2.52 & 21.00 & 6.54 & 87.86 (65.33) & 86.91 & 87.82\\
       BERTweet\textsubscript{large}    &  25.76 & 48.98 & 14.12 & 87.68 (75.14) & 89.03 & 86.34 & 4.24 & 25.68 & 9.49 & 88.88 (68.89) & 87.80 & 88.16 \\
       \cmidrule{1-13}
       \textit{Fine-tune on ParaNMT} \\
       BERT\textsubscript{large}-random-init. & 7.95 & 33.12 & 7.61 & 83.33 (65.90) & 83.37 & 83.98 & 11.07 & 35.16 & 12.88 & 91.25 (76.73) & 90.41 & 88.85\\
        BERT\textsubscript{large} & 18.11 & 45.94 & 17.49 & 89.13 (77.91) & 88.42 & 85.88 & 13.32 & 39.25 & 14.51 & 92.17 (79.80) & 91.60 & 88.89 \\   
       BERTweet\textsubscript{large}   &  19.29 & 48.00 & 20.39 & 90.00 (79.63) & 89.04 & 86.85 & 15.63 & 40.71 & 16.75 & 92.40 (80.10) & 91.86 & 88.78  \\
        \bottomrule
\end{tabular}}
\caption{Fine-tune on $M_{\alpha} + M^{New}_{\beta}$, evaluate on \dataset-NMR \wx{use a more intuitive name than $M_{\alpha} + M^{New}_{\beta}$}}
\label{table:encoder_decoder}
\end{table*}

==> fig/generation_dataset_comparison_old.tex <==
\setlength{\tabcolsep}{3pt}
\begin{table*}[t]
    \centering
    {\renewcommand{\arraystretch}{1.25}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{@{}lccccccc|ccccc|ccccc|ccccc@{}}
        \toprule
         \multicolumn{3}{c}{\textit{Test set \rightarrow}} & \multicolumn{5}{c}{\textbf{MultiPIT-NMR}} & \multicolumn{5}{c}{\textbf{Quora}} & \multicolumn{5}{c}{\textbf{MSCOCO}} &
         \multicolumn{5}{c}{\textbf{ParaNMT}}
            \\ \cmidrule(r){4-8} \cmidrule(r){9-13} \cmidrule(r){14-18} \cmidrule(r){19-23}
       \multicolumn{2}{l}{\textit{{Training set}}} & & BL & R-L & S-B $\downarrow$ & B-S & B-iB & BL & R-L & S-B $\downarrow$ & B-S & B-iB & BL & R-L & S-B $\downarrow$ & B-S & B-iB & BL & R-L & S-B $\downarrow$ & B-S & B-iB\\ 
       \midrule
            &
            \multicolumn{1}{l}{M + M-New (filtered)} & & \textbf{44.56} & \textbf{61.00} & 31.85 & \textit{85.25} & \textbf{78.14} &  20.99 & 50.55 & 37.39 & \textit{88.84} & 70.82 & \textit{17.85} & 43.60 & 41.84 & \textit{89.07} & 75.05 & \textit{13.22} & \textit{35.24} & 40.27 & \textit{84.33} & 71.19\\
           & \multicolumn{1}{l}{\textbf{Quora}} & & 33.36 & 55.81 & \textit{31.76} & 83.32 & 76.88 & \textbf{26.87} & \textbf{60.42} & \textit{34.85} & 88.11 & \textit{72.53} & 16.51 & 42.50 & 51.03 & 88.78 & 67.16 & 9.76 & 33.24 & \textit{25.21} & 78.21 & \textit{71.49}\\
           & \multicolumn{1}{l}{\textbf{MSCOCO}} & & 4.05 & 17.16 & \textbf{1.95} & 58.11 & 62.94 & 0.88 & 8.97 & \textbf{1.10} & 58.03 & 62.99 & \textbf{23.85} & \textbf{50.99} & \textbf{11.66} & 80.44 & \textbf{81.03} & 0.49 & 7.38 & \textbf{0.51} & 57.27 & 62.22 \\
           & \multicolumn{1}{l}{\textbf{ParaNMT}} & & \textit{38.65} & \textit{58.12} & 41.11 & \textbf{88.57} & \textit{76.95} & \textit{22.77} & \textit{56.89} & 39.00 & \textbf{90.04} & \textbf{73.84} & 16.62 & \textit{44.01} & \textit{36.30} & \textbf{90.09} & \textit{80.22} & \textbf{18.35} & \textbf{43.70} & 26.33 & \textbf{85.00} & \textbf{78.28}\\
        %   & \multicolumn{1}{l}{\textbf{ParaNMT}} & & 36.65 & 57.78 & 38.57 & \textbf{88.44} & 77.36 & 22.16 & 56.31 & 37.92 & \textbf{89.95} & \textbf{75.25} & 16.10 & 43.14 & 35.69 & \textbf{90.31} & 80.64 & \textbf{18.86} & \textbf{44.13} & 25.63 & \textbf{84.70} & \textbf{78.96}\\
        \bottomrule
    \end{tabular}
    }}
    \caption{Automatic evaluation of models fine-tuned on four datasets. Here, BL : BLEU, R-L : ROUGE-L, S-B : Self-BLEU, B-S : BERT-Score, B-iB : BERT-iBLEU. \textbf{Bold}: the best, \textit{Italic}: the second best.}
    \label{table:generation_dataset_comparison}
\end{table*}

==> fig/generation_dataset_comparison_old_v2.tex <==
\setlength{\tabcolsep}{3pt}
\begin{table*}[t]
    \centering
    {\renewcommand{\arraystretch}{1.25}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{@{}lccccccc|ccccc|ccccc|ccccc@{}}
        \toprule
         \multicolumn{3}{c}{\textit{Test set \rightarrow}} & \multicolumn{5}{c}{\textbf{MultiPIT-NMR}} & \multicolumn{5}{c}{\textbf{Quora}} & \multicolumn{5}{c}{\textbf{MSCOCO}} &
         \multicolumn{5}{c}{\textbf{ParaNMT}}
            \\ \cmidrule(r){4-8} \cmidrule(r){9-13} \cmidrule(r){14-18} \cmidrule(r){19-23}
       \multicolumn{2}{l}{\textit{{Training set}}} & & BL & R-L & S-B $\downarrow$ & B-S & B-iB & BL & R-L & S-B $\downarrow$ & B-S & B-iB & BL & R-L & S-B $\downarrow$ & B-S & B-iB & BL & R-L & S-B $\downarrow$ & B-S & B-iB\\ 
       \midrule
            &
            \multicolumn{1}{l}{$M_{\alpha} + M^{New}_{\beta}$ (M)} & & \textbf{44.56} & \textbf{61.00} & 31.85 & \textbf{92.00} & \textit{84.53} &  20.99 & 50.55 & 37.39 & \textit{88.84} & 70.82 & \textit{17.85} & 43.60 & 41.84 & \textit{89.07} & 75.05 & \textit{13.22} & \textit{35.24} & 40.27 & \textit{84.33} & 71.19\\
           & \multicolumn{1}{l}{\textbf{Quora}} & & 33.36 & 55.81 & \textit{31.76} & 
          \textit{90.96} & 84.06 & \textbf{26.87} & \textbf{60.42} & \textit{34.85} & 88.11 & \textit{72.53} & 16.51 & 42.50 & 51.03 & 88.78 & 67.16 & 9.76 & 33.24 & \textit{25.21} & 78.21 & \textit{71.49}\\
           & \multicolumn{1}{l}{\textbf{MSCOCO}} & & 4.05 & 17.16 & \textbf{1.95} & 81.25 & 83.38 & 0.88 & 8.97 & \textbf{1.10} & 58.03 & 62.99 & \textbf{23.85} & \textbf{50.99} & \textbf{11.66} & 80.44 & \textbf{81.03} & 0.49 & 7.38 & \textbf{0.51} & 57.27 & 62.22 \\
           & \multicolumn{1}{l}{\textbf{ParaNMT}} & & 38.65 & \textit{58.12} & 41.11 & 91.69 & 81.97 & \textit{22.77} & \textit{56.89} & 39.00 & \textbf{90.04} & \textbf{73.84} & 16.62 & \textit{44.01} & \textit{36.30} & \textbf{90.09} & \textit{80.22} & \textbf{18.35} & \textbf{43.70} & 26.33 & \textbf{85.00} & \textbf{78.28}\\
           & \multicolumn{1}{l}{\textbf{M + ParaNMT}} & & \textit{39.07} & 57.80 & 25.80 & 91.58 & \textbf{87.25} \\
        %   & \multicolumn{1}{l}{\textbf{ParaNMT}} & & 36.65 & 57.78 & 38.57 & \textbf{88.44} & 77.36 & 22.16 & 56.31 & 37.92 & \textbf{89.95} & \textbf{75.25} & 16.10 & 43.14 & 35.69 & \textbf{90.31} & 80.64 & \textbf{18.86} & \textbf{44.13} & 25.63 & \textbf{84.70} & \textbf{78.96}\\
        \bottomrule
    \end{tabular}
    }}
    \caption{Automatic evaluation of models fine-tuned on four datasets. Here, BL : BLEU, R-L : ROUGE-L, S-B : Self-BLEU, B-S : BERT-Score, B-iB : BERT-iBLEU. \textbf{Bold}: the best, \textit{Italic}: the second best.}
    \label{table:generation_dataset_comparison}
\end{table*}

==> fig/generation_main.tex <==
\setlength{\tabcolsep}{3pt}
\begin{table*}[h]
\centering
\renewcommand{\arraystretch}{1.25}
\resizebox{0.85\textwidth}{!}{
\begin{tabular}{@{}lcccccc|cccc|cccc|cccc@{}}
\toprule
     \multicolumn{3}{c}{\textit{Training set \rightarrow}} & \multicolumn{4}{c}{\textbf{\textit{MultiPIT}}} & \multicolumn{4}{c}{\textbf{\textit{Quora}}} & \multicolumn{4}{c}{\textbf{\textit{MSCOCO}}} &
     \multicolumn{4}{c}{\textbf{\textit{ParaNMT}}}
        \\ \cmidrule(r){4-7} \cmidrule(r){8-11} \cmidrule(r){12-15} \cmidrule(r){16-19}
   \multicolumn{2}{l}{\textbf{Model}} &  & \textbf{B-4} & \textbf{R-L} & \textbf{S-B} $\downarrow$ & \textbf{B-S} &   \textbf{B-4} & \textbf{R-L} & \textbf{S-B} $\downarrow$ & \textbf{B-S}  &  \textbf{B-4} & \textbf{R-L} & \textbf{S-B} $\downarrow$ & \textbf{B-S}  &  \textbf{B-4} & \textbf{R-L} & \textbf{S-B} $\downarrow$ & \textbf{B-S}\\ 
   \midrule
       \multicolumn{2}{l}{GPT-2${_{small}}$}    &
       \multirow{7}{*}{\rotatebox[origin=c]{90}{Macro Average}}  & \\
    \multicolumn{2}{l}{GPT-2${_{large}}$}      &   \\
   \multicolumn{2}{l}{ BART${_{base}}$}      &    \\
    \multicolumn{2}{l}{BART${_{large}}$}   &   \\
    \multicolumn{2}{l}{T5${_{small}}$}     &    \\
    \multicolumn{2}{l}{T5${_{base}}$}     & \\
    \multicolumn{2}{l}{T5${_{large}}$ \downarrow}  &  & 21.93 & 52.27 & 46.16 & 87.44 & 22.86 & 53.12 & 67.45 & 93.14 & 7.92 & 22.44 & 6.64 & 64.32 & 13.65 & 48.08 & 20.89 & 84.67 \\ \midrule
       \multicolumn{1}{l}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Test set}}} &
        \multicolumn{1}{c}{\textbf{\textit{MultiPIT}}} & \multirow{4}{*}{\rotatebox[origin=c]{90}{Individual}} & 32.68 & 62.31 & 43.57 & 84.94 & 22.27 & 58.15 & 52.45 & 88.72 & 2.34 & 15.56 & 2.02 & 57.86 & 9.28 & 48.76 & 13.21 & 79.52  \\
       & \multicolumn{1}{c}{\textbf{\textit{Quora}}} & & 25.73 & 60.45 & 52.52 & 90.89 & 35.50 & 65.75 & 56.19 & 92.29 & 1.11 & 11.91 & 1.43 & 58.65 & 13.15 & 51.33 & 22.04 & 87.02  \\
       & \multicolumn{1}{c}{\textbf{\textit{MSCOCO}}} & & 18.17 & 47.65 & 48.13 & 89.77 & 18.51 & 47.76 & 92.35& 98.37 & 27.64 & 54.33 & 22.28 & 83.28 & 13.79 & 43.69 & 27.84 & 88.79 \\
       & \multicolumn{1}{c}{\textbf{\textit{ParaNMT}}} & & 11.14 & 38.67 & 40.43 & 84.19 &  15.16 & 40.82 & 68.83 & 93.17 & 0.58 & 7.96 & 0.84 & 57.51 & 18.37 & 48.55 & 20.47 & 83.35\\
    \bottomrule
\end{tabular}}
\caption{Comparison of results of different transformer models fintetuned on all three datasets, the metric are averaged, \textbf{Topic} part of \datasetname, and \textbf{URL} part of \datasetname. 4 Nvidia A40 GPU were used for this experiment. Each setup was trained for 3 epochs and the best epoch performance was reported.}
\label{table:generation_main}
\end{table*}

==> fig/generation_main_v2.tex <==
\setlength{\tabcolsep}{3pt}
\begin{table*}[h]
\centering
\renewcommand{\arraystretch}{1.25}
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{@{}lcccccc|cccc|cccc|cccc@{}}
\toprule
     \multicolumn{3}{c}{\textit{Training set \rightarrow}} & \multicolumn{4}{c}{\textbf{MultiPIT}} & \multicolumn{4}{c}{\textbf{Quora}} & \multicolumn{4}{c}{\textbf{MSCOCO}} &
     \multicolumn{4}{c}{\textbf{ParaNMT}}
        \\ \cmidrule(r){4-7} \cmidrule(r){8-11} \cmidrule(r){12-15} \cmidrule(r){16-19}
   \multicolumn{2}{l}{\textbf{Models}} &  & B-4 & R-L & S-B $\downarrow$ & B-S & B-4 & R-L & S-B $\downarrow$ & B-S & B-4 & R-L & S-B $\downarrow$ & B-S  &   B-4 & R-L & S-B $\downarrow$ & B-S\\ 
   \midrule
       \multicolumn{19}{l}{\textit{Averaged performance over four testsets}} \\ \midrule

   
       \multicolumn{2}{l}{GPT-2${_{small}}$}    &
         & \\
    \multicolumn{2}{l}{GPT-2${_{large}}$}      &  & 5.90 & 28.98 & 9.63 & 66.67 & 11.15 & 37.30 & 24.53 & 75.58 & 3.07 & 15.81 & 2.03 & 59.65 & 5.42 & 33.06 & 6.69 & 73.82 \\
   \multicolumn{2}{l}{ BART${_{base}}$}      &    \\
    \multicolumn{2}{l}{BART${_{large}}$}   &  & 22.55 & 51.75 & 48.61 & 88.16 & 22.76 & 51.45 & 66.84 & 90.31 & 8.57 & 22.00 & 7.55 & 63.74 & 12.70 & 44.94 & 18.05 & 83.72  \\
    \multicolumn{2}{l}{T5${_{small}}$}     &    \\
    \multicolumn{2}{l}{T5${_{base}}$}     & \\
    \multicolumn{2}{l}{T5${_{large}}$}  &  & 21.93 & 52.27 & 46.16 & 87.44 & 22.86 & 53.12 & 67.45 & 93.14 & 7.92 & 22.44 & 6.64 & 64.32 & 13.65 & 48.08 & 20.89 & 84.67 \\ \midrule
    
    \multicolumn{19}{l}{\textit{Performance of T5$_{large}$ model on different testsets}} \\ \midrule
    
        &
        \multicolumn{1}{l}{\textbf{MultiPIT}} & \multirow{4}{*}{\rotatebox[origin=c]{90}{}} & 32.68 & 62.31 & 43.57 & 84.94 & 22.27 & 58.15 & 52.45 & 88.72 & 2.34 & 15.56 & 2.02 & 57.86 & 9.28 & 48.76 & 13.21 & 79.52  \\
       & \multicolumn{1}{l}{\textbf{Quora}} & & 25.73 & 60.45 & 52.52 & 90.89 & 35.50 & 65.75 & 56.19 & 92.29 & 1.11 & 11.91 & 1.43 & 58.65 & 13.15 & 51.33 & 22.04 & 87.02  \\
       & \multicolumn{1}{l}{\textbf{MSCOCO}} & & 18.17 & 47.65 & 48.13 & 89.77 & 18.51 & 47.76 & 92.35& 98.37 & 27.64 & 54.33 & 22.28 & 83.28 & 13.79 & 43.69 & 27.84 & 88.79 \\
       & \multicolumn{1}{l}{\textbf{ParaNMT}} & & 11.14 & 38.67 & 40.43 & 84.19 &  15.16 & 40.82 & 68.83 & 93.17 & 0.58 & 7.96 & 0.84 & 57.51 & 18.37 & 48.55 & 20.47 & 83.35\\
    \bottomrule
\end{tabular}}
\caption{Comparison of results of different transformer models fintetuned on all three datasets, the metric are averaged, \textbf{Topic} part of \datasetname, and \textbf{URL} part of \datasetname. 4 Nvidia A40 GPU were used for this experiment. Each setup was trained for 3 epochs and the best epoch performance was reported.}
\label{table:generation_main}
\end{table*}

==> fig/generation_model_comparison.tex <==
\begin{table}[t]
\centering
\renewcommand{\arraystretch}{1.05}
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{@{}lcccccc@{}}
\toprule
%   \textbf{Model} & BLEU & ROUGE-L & Self-BLEU & BERT-Score & BERT-iBLEU  \\ 
   \textbf{Model} & \#Para. & LR & BL & S-B $\downarrow$ & B-S & B-iB  \\ 
   \midrule
   
      GPT-2\textsubscript{small}   & 117M & 1e-4 & 44.01 & 82.93 & \textbf{95.08} & 35.60  \\ % 1e-4
    GPT-2\textsubscript{large}   & 774M  & 1e-4  & 43.94 & 70.14 & 92.19 & 54.45 \\ % 1e-4
   BART\textsubscript{base}  & 139M  & 1e-5 &  46.47 & 68.07 & 92.24 & 52.74  \\ % 1e-5 seed 12
    % BART\textsubscript{large}   & \textbf{46.03} & \textbf{61.18} & \textbf{62.07} & 90.83 & 61.11 \\ % 1e-5
    BART\textsubscript{large} & 406M & 1e-5 & \textbf{47.66} & 66.50 & 91.76 & 57.95 \\ % 1e-5 seed 12
    T5\textsubscript{small} & 60M  & 3e-4   & 44.78 & 80.12 & 95.15 & 40.73  \\ % 3e-4
    T5\textsubscript{base}  & 220M  & 1e-4 & 45.00 & 70.07 & 92.39 & 54.76 \\ % 1e-4
    T5\textsubscript{large} & 770M & 1e-4 &  45.85 & \textbf{65.03} & 91.86 & \textbf{59.87} \\ % 1e-4
    \bottomrule
\end{tabular}}
\caption{Test set results of different transformer models fine-tuned on \newdata. Here, BL: BLEU, S-B: Self-BLEU, B-S: BERT-Score, B-iB: BERT-iBLEU. LR denotes learning rate.
We tune the learning rate for each model on the dev set and report the best one.}
\vspace{-10pt}
\label{table:generation_model_comparison}
\end{table}

% Both BART\textsubscript{large} and T5\textsubscript{large} perform competitively with the highest BLEU and highest BERT-iBLEU, respectively.

==> fig/generation_model_comparison_old.tex <==
\begin{table}[t]
\centering
% \renewcommand{\arraystretch}{1.2}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}lccccc@{}}
\toprule
   \textbf{Model} & BLEU & ROUGE-L & self-BLEU & BERT-Score & BERT-iBLEU  \\ 
   \midrule
   
      GPT-2\textsubscript{small}   & 8.64 & 31.47 & 12.22 & 64.63 & 66.64\\
    GPT-2\textsubscript{large}      & 9.75 & 35.51 & 10.59 & 67.11 & 69.41 \\
   BART\textsubscript{base}     &  34.19 & 63.65 & 53.21 & 87.30 & 63.44  \\
    BART\textsubscript{large}   & 32.96 & 61.57 & 44.90 & 84.53 & 67.98 \\
    T5\textsubscript{small}      & 42.74 & 59.20 & 78.19 & 94.81 & 43.05  \\ % 3e-4 need to rerun for old
    T5\textsubscript{base}     & 43.30 & 60.10 & 68.48 & 92.01 & 55.68 \\ % 1e-4 need to rerun for old
    T5\textsubscript{large}  &  44.18 & 60.74 & 63.05 & 91.51 & 62.33 \\ % 1e-4 need to rerun for old
    \bottomrule
\end{tabular}}
\caption{Performance of different transformer models fine-tuned on Multipit. T5\textsubscript{large} performs the best with high enough BERT-Score and low self-BLEU among all models.}
\label{table:generation_main}
\end{table}

==> fig/generation_setup_comparison.tex <==
\begin{table*}[t]
\centering
\renewcommand{\arraystretch}{1.2}
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}lrrrrrr@{}}
\toprule
   \textbf{Data} & Size & BLEU-4 & ROUGE-L & SELF-BLEU & BERT-Score & BERT-iBLEU  \\ 
   \midrule
     Multipit  & 50001 & 32.68 & 62.31& 43.57 & 84.94 & 68.58\\
    M (B-4 $\leq 10$)  & 18844 & 25.09 & 59.47 & 28.14 & 82.03 & 74.97 \\
    M (B-4 $\leq 20$)    & & 26.31 & 59.30 & 30.66 & 82.19 & 74.15\\
    New Trend & & \\
    New URL & & \\
    M + New Trend & & \\
    M + New URL & \\
    M + New Trend and URL & & 30.26 & 58.42 & 44.64 & 83.19 & 70.06\\
    M (B-4 $\leq 10$) + New (B-4 $\leq 10$)   & & 20.56 & 53.75 & 19.90 & 78.14 & 76.99\\
    M (B-4 $\leq 10$) + New (B-4 $\leq 10$ \& B-S $\geq 75$)   &  & 25.45 & 59.94 & 27.53 & 83.45 & 78.03\\
    Oversample(M (B-4 $\leq 10$) + New (B-4 $\leq 10$ \& B-S $\geq 75$))  & & 24.20 & 58.89 & 23.89 & 82.70 & 79.11\\
    \bottomrule
\end{tabular}}
\caption{Performance of T5 model fintetuned on several Multipit data setups. Models are evaluated on the Multipit test set.}
\label{table:generation_setup_comparison}
\end{table*}

==> fig/human_evaluation_old.tex <==
\setlength{\tabcolsep}{3pt}
\begin{table*}[h]
\centering
\renewcommand{\arraystretch}{1.25}
\begin{minipage}[t]{.32\linewidth}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}lcccc@{}}
\toprule
 \textbf{Models} & \textbf{Fluency} & \multicolumn{1}{p{2.4cm}}{\centering \textbf{Semantic Similarity}}  & \textbf{Diversity}  & \multicolumn{1}{p{2.4cm}}{\centering \textbf{Number of Annotations}} \\
 \midrule
 \textbf{MultiPIT} & \textbf{4.88} & 4.23 & 2.55 & 199 \\
 \textbf{Quora} &  4.87  & \textbf{4.68} & 1.77 & 199\\
\textbf{MSCOCO} & 4.87 & 2.02 & \textbf{4.60} & 200 \\
\textbf{ParaNMT} & 4.75 & 4.12 & 3.11 & 199\\
\bottomrule
\end{tabular}}
\captionof{table}{First round (one annotation per pair) Human evaluation result for models finetuned on the four datasets.}
\end{minipage}
\hfill
\begin{minipage}[t]{.32\linewidth}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}lcccc@{}}
\toprule
 \textbf{Models} & \textbf{Fluency} & \multicolumn{1}{p{2.4cm}}{\centering \textbf{Semantic Similarity}}  & \textbf{Diversity}  & \multicolumn{1}{p{2.4cm}}{\centering \textbf{Number of Annotations}} \\
 \midrule
 \textbf{MultiPIT} & \textbf{4.88} & 4.09 & 2.83 & 168 \\
 \textbf{Quora} &  4.79  & \textbf{4.26} & 2.77 & 87\\
\textbf{MSCOCO} & 4.87 & 2.00 & \textbf{4.62} & \textbf{199} \\
\textbf{ParaNMT} & 4.74 & 4.08 & 3.18 & 192\\
\bottomrule
\end{tabular}}
\captionof{table}{Remove the pairs that generation directly copy the source sentence (ignoring lettercase and punctuation). (Diversity != 1)}
\end{minipage}
\hfill
\begin{minipage}[t]{.32\linewidth}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}lcccc@{}}
\toprule
 \textbf{Models} & \textbf{Fluency} & \multicolumn{1}{p{2.4cm}}{\centering \textbf{Semantic Similarity}}  & \textbf{Diversity}  & \multicolumn{1}{p{2.4cm}}{\centering \textbf{Number of Annotations}} \\
 \midrule
 \textbf{MultiPIT} & 4.92 & 4.63 & 2.15 & 153 \\
 \textbf{Quora} &  4.88  & \textbf{4.82} & 1.61 & \textbf{185}\\
\textbf{MSCOCO} & \textbf{4.96} & 4.19 & \textbf{3.12} & 26 \\
\textbf{ParaNMT} & 4.82 & 4.49 & 2.93 & 157\\
\bottomrule
\end{tabular}}
\captionof{table}{Select pairs that has semantic similarity $> 3$.}
\end{minipage}
\label{table:human_evaluation}
\end{table*}

==> fig/identification_main.tex <==
% \setlength{\tabcolsep}{3pt}
\begin{table*}[h]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccc|cccc|cccc|cccc}
\toprule
     \multicolumn{3}{c}{\textit{Training set \rightarrow}} & \multicolumn{4}{c}{\textbf{\textit{MultiPIT}}} & \multicolumn{4}{c}{\textbf{\textit{Quora}}} & \multicolumn{4}{c}{\textbf{\textit{MRPC}}} & \multicolumn{4}{c}{\textbf{\textit{PAWS}}}
    \\ \cmidrule(r){4-7} \cmidrule(r){8-11} \cmidrule(r){12-15} \cmidrule(r){16-19}
   \multicolumn{2}{l}{\textbf{Model}} &  &  \textbf{P} & \textbf{R} &\textbf{F} & \textbf{Acc} &  \textbf{P} & \textbf{R} &\textbf{F} & \textbf{Acc} &  \textbf{P} & \textbf{R} &\textbf{F} & \textbf{Acc} &  \textbf{P} & \textbf{R} &\textbf{F} & \textbf{Acc}   \\ 
   \midrule 
    \multicolumn{2}{l}{BERT${_{base}}$}   & \multirow{7}{*}{\rotatebox[origin=c]{90}{Macro Average}}  &     \\
    \multicolumn{2}{l}{BERT${_{large}}$}    &    &   \\
    \multicolumn{2}{l}{DEBERTA${_{large}}$}    &  &      \\
    \multicolumn{2}{l}{DEBERTA${_{xlarge}}$} &  &  \\
    \multicolumn{2}{l}{T5${_{small}}$}   &    &    \\
    \multicolumn{2}{l}{T5${_{base}}$}   &   & \\
    \multicolumn{2}{l}{T5${_{large}}$}  &     &  \\
    \midrule
       \multicolumn{3}{c}{\textit{Test set \downarrow}} \\
       \multicolumn{1}{l}{\multirow{4}{*}{\rotatebox[origin=c]{90}{T5${_{large}}$}}} &
        \multicolumn{1}{c}{\textbf{\textit{MultiPIT}}} & \multirow{4}{*}{\rotatebox[origin=c]{90}{Individual}} & 90.2 & 93.4 & 91.7 & 91.0 & 82.1 & 82.3 & 82.2 & 80.9 & 88.7 & 77.1 & 82.5 & 82.5 & 91.7 & 59.7 & 72.3 & 75.5\\
       & \multicolumn{1}{c}{\textbf{\textit{Quora}}} & & 65.4 & 91.4 & 76.3 & 78.9 & 87.5 & 91.0 & 89.2 & 91.9 & 68.3 & 84.9 & 75.7 & 79.8 & 77.4 & 70.1 & 73.6 & 81.4 \\
       & \multicolumn{1}{c}{\textbf{\textit{MRPC}}} & & 72.0 & 99.5 & 83.5 & 73.9 & 76.6 & 76.8 & 76.7 & 69.0 & 89.6 & 95.0 & 92.3 & 89.4 & 87.5 & 70.8 & 78.3 & 73.9 \\
       & \multicolumn{1}{c}{\textbf{\textit{PAWS}}} & & 44.2 & 100 & 63.3 & 44.2 & 53.0 & 96.2 & 68.3 & 60.5 & 44.5 & 99.9 & 61.5 & 44.8 & 92.4 & 95.8 & 94.1 & 94.7\\
    \bottomrule
\end{tabular}}
\caption{Comparison of results of different transformer models fintetuned on \datasetname, Quora, MRPC, PAWS dataset.}
\label{table:identification_main}
\end{table*}

==> fig/identification_main_V2.tex <==
% \setlength{\tabcolsep}{3pt}

 \aboverulesep=0ex
 \belowrulesep=0ex
\begin{table*}[h]
\renewcommand{\arraystretch}{1.25}
\small
\centering
% \resizebox{0.7\textwidth}{!}{
\begin{tabular}{L{2.3cm}|C{1cm}C{0.9cm}|C{1.25cm}C{0.95cm}C{0.95cm}C{0.95cm}C{0.95cm}|C{1.25cm}C{0.95cm}C{0.95cm}C{0.95cm}}
% \begin{tabular}{p{2cm} p{2cm}p{2cm}p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}}


\toprule


\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\#Para.}  & \multirow{2}{*}{LR.} & \multicolumn{5}{c|}{\textbf{MultiPIT Test Set}} & \multicolumn{4}{c}{\textbf{Latest Testset}} \\
 
 & & & Precision & Recall & F1 & Acc. & Speed & Precision & Recall & F1 & Acc. \\

% \textbf{Precision} & \textbf{Recall} &\textbf{F1} & \textbf{Acc.} &  \textbf{Speed} & \textbf{F1}$_{new}$  \\ 
   \midrule
   ESIM & 17M & 1e-4 & 88.43 & 74.83 & 81.07 & 83.79 &  4.9s & -&-&-&- \\

    Infersent & 47M & 1e-5 & 88.18 & 88.21 &88.19 & 87.34 & 3.2s & -&-&-&- \\
    \midrule
    BERT\textsubscript{base}    & 109M   &  5e-5 & 89.02 & 91.87 & 90.42 & 89.57 & 11.4s& -&-&-&-\\
    BERT\textsubscript{large}    & 335M   &  5e-5 & 90.06 & 92.46 & 91.25 & 90.49 & 26.8s& -&-&-&-\\
    RoBERTa\textsubscript{large} &  355M & 2e-5 & 88.94 & 95.31 & 92.01 & 91.13 & 29.1s& -&-&-&-\\
    DeBERTa\textsubscript{large-v3}    & 400M &   8e-6 & 89.41 & 95.21 & \textbf{92.22} & \textbf{91.38}  & 37.1s& -&-&-&-\\
    DeBERTa\textsubscript{xlarge-v2} & 900M & 8e-6  & 90.66 & 93.27 & 91.95 & 91.24 & 65.8s & -&-&-&-\\
    ALBERT\textsubscript{xxlarge-v2}   & 235M   &  2e-5 & \textbf{91.59} & 92.03 & 91.81 & 91.19 & 63.2s& -&-&-&- \\
      T5\textsubscript{base}   & 220M  & 1e-4 & 87.53 & \textbf{95.52} & 91.35 & 90.30 & 32.9s &  -&-&-&-\\
    T5\textsubscript{large}  &   770M  & 1e-4 & 89.00 & 94.76 & 91.79 & 90.91 & 84.1s& -&-&-&- \\ 
    \bottomrule
\end{tabular}
% }
\caption{Evaluation results on the test set of MultiPIT and a new testset with up-to-date data. LR. denotes learning rate, and Speed is measured by second per sentence pair. All transformer-based models are finetuned with 32 batch size for 3 epochs on 4 Nivida A40 GPUs. Infersent and ESIM are trained on 1 GPU with 64/32 batch size. The epoch with highest precision on dev set are used for evaluation, as the models will be mainly used for extracting  paraphrase pairs from unlabeled data. }
\label{table:identification_main_v2}
\end{table*}

==> fig/identification_methods_comparison.tex <==
% \setlength{\tabcolsep}{3pt}

 \aboverulesep=0ex
 \belowrulesep=0ex
\begin{table*}[h]
\renewcommand{\arraystretch}{1.25}
\small
\centering
% \resizebox{0.7\textwidth}{!}{
\begin{tabular}{lcccccccc}

\toprule
   \textbf{Model} & \textbf{\#Para.} & \textbf{LR} & \textbf{Precision} & \textbf{Recall} &\textbf{F1} & \textbf{Acc.} & \textbf{Speed} & \textbf{F1}$_{new}$  \\ 
   \midrule
   

    BERT\textsubscript{base}    & 109M   &  5e-5 & 89.02 & 91.87 & 90.42 & 89.57 & 11.4s&\\
    BERT\textsubscript{large}    & 335M   &  5e-5 & 90.06 & 92.46 & 91.25 & 90.49 & 26.8s&\\
    RoBERTa\textsubscript{large} &  355M & 2e-5 & 88.94 & 95.31 & 92.01 & 91.13 & 29.1s& \\
    DeBERTa\textsubscript{large-v3}    & 400M &   8e-6 & 89.41 & 95.21 & \textbf{92.22} & \textbf{91.38}  & 37.1s&\\
    DeBERTa\textsubscript{xlarge-v2} & 900M & 8e-6  & 90.66 & 93.27 & 91.95 & 91.24 & 65.8s &\\
    ALBERT\textsubscript{xxlarge-v2}   & 235M   &  2e-5 & \textbf{91.59} & 92.03 & 91.81 & 91.19 & 63.2s& \\
       T5\textsubscript{base}   & 220M  & 1e-4 & 87.53 & \textbf{95.52} & 91.35 & 90.30 & 32.9s & \\
    T5\textsubscript{large}  &   770M  & 1e-4 & 89.00 & 94.76 & 91.79 & 90.91 & 84.1s& \\
    \midrule
    Infersent &&&&&&&& \\
   ESIM &&&&&&&& \\
    \bottomrule
\end{tabular}
% }
\caption{Test set results for different transformer models finetuned on \datasetname.}
\label{table:identification_main_v2}
\end{table*}

==> fig/paraphrase_definition_examples.tex <==
\begin{table}[t]
\centering
\renewcommand{\arraystretch}{1.2}
\resizebox{0.49\textwidth}{!}{
\begin{tabular}{lcc}
\toprule
Sentence Pair & Iden. & Gen. \\
\midrule
S1: Buccaneers' Antonio Brown suspended 3 games for COVID-19 violation. & \multirow{2}{*}{\ding{51}} & \multirow{2}{*}{\ding{55}} \\
S2: NFL suspends Antonio Brown three games over fake vaccination card. & & \\
\midrule
S1: All three men involved in the killing of Ahmaud Arbery found guilty of murder. & \multirow{2}{*}{\ding{51}} & \multirow{2}{*}{\ding{55}} \\
S2: Georgia jury convicts three white men of murder in the death of Ahmaud Arbery. & &\\
\bottomrule
\end{tabular}}
\caption{Different paraphrase criteria for identification and generation. In both examples, S1 and S2 are about the same subject.
% : suspension of Antonio Brown and conviction of killers in Ahmaud Arbery's murder respectively. 
However, both S2 introduce new information that requires further context: fake vaccination card, and Georgia jury and white men. Here, Iden. represents Identification, and Gen. represents Generation.}
\label{table:paraphrase_definition_examples}
\end{table}
